Information-theoretic limits of a multiview low-rank symmetric spiked matrix model

We consider a generalization of an important class of high-dimensional inference problems, namely spiked symmetric matrix models, often used as probabilistic models for principal component analysis. Such paradigmatic models have recently attracted a lot of attention from a number of communities due to their phenomenological richness with statistical-to-computational gaps, while remaining tractable. We rigorously establish the information-theoretic limits through the proof of single-letter formulas for the mutual information and minimum mean-square error. On a technical side we improve the recently introduced adaptive interpolation method, so that it can be used to study low-rank models (i.e., estimation problems of "tall matrices") in full generality, an important step towards the rigorous analysis of more complicated inference and learning models.

==> sections/proof.tex <==

We give here the main steps of the proof of Theorem~\ref{thm:main_thm}. We will use the adaptive interpolation method, introduced in \cite{barbier_stoInt}, and then applied in \cite{2017arXiv170910368B} and \cite{Barbier2017}. It is a powerful evolution of the interpolation method developed by Guerra and Toninelli in the context of spin glasses \cite{guerra2002thermodynamic}. Many steps of the proof follow the ones of \cite{Barbier2017}, and we will refer to them when necessary.

% \subsection{Key idea}

% The key point of such the decomposition Eq.\ref{eq:decomposition} is to be able to relate the $\cal R$-transform of $\frac{1}{n}\bm{\Phi}^\intercal\bm{\Phi}$ and the so-called Shannon transform \cite{2004random} of $\frac{1}{n}\bm{\Phi'}^\intercal\bm{\Phi'}$. Such a relation is described for instance in \cite{0911.0087}. More precisely, when the following quantities are well defined (as a function of $z$), one has : 
% \begin{align}\label{eq:link_r_shannon}
%  \mathcal{R}_{\frac{1}{n}\bm{\Phi}^\intercal \bm{\Phi}}(-z) = \mathbb{E}_{X \sim \frac{1}{n}\bm{\Phi'}^\intercal \bm{\Phi'}} \left[\frac{X}{1+X z}\right]
% \end{align}
% In which the abusive notation $X \sim \frac{1}{n}\bm{\Phi'}^\intercal \bm{\Phi'}$ means that $X$ follows the asymptotic eigenvalue distribution of $\frac{1}{n}\bm{\Phi'}^\intercal \bm{\Phi'}$.

% The intuition that drove us to Eq.\ref{eq:link_r_shannon} was motivated by the remark that the simple construction Eq.\ref{eq:decomposition} implies that the asymptotic eigenvalue distribution of $\frac{1}{n}\bm{\Phi}^\intercal \bm{\Phi}$ is constructed as a \emph{free compound Poisson distribution} \cite{0911.0087},\cite{nica2006lectures} with jump distribution given by the asymptotic eigenvalue distribution of $\frac{1}{n}\bm{\Phi'}^\intercal \bm{\Phi'}$. 

\subsection{Interpolating estimation problem}

Let $E : [0,1] \to \mathbb{R}_+$ be a continuous ``interpolation function'', $r \geq 0$ and $t\in[0,1]$. Define $\widetilde E(t)\equiv \int_0^t E(s)ds$ (and thus $\widetilde E'(t)=E(t)$), that plays the role of a signal-to-noise ratio. Assume one has access to the following two $t$-dependent observation channels for $i=1,\ldots,n$ and $\mu=1,\ldots,m$:

\begin{align}
	\begin{cases}
	Y_{t,\mu} &= \sqrt{\frac{\lambda(1-t)}{n}}(\bm{\Phi} \bX)_\mu+ \sqrt{\frac{\lambda}{n} \widetilde E(t)} (\bm{\Phi'} \bV)_\mu  + Z_\mu\,,\\
	\widetilde Y_{t,i} &= \sqrt{rt} X_i + \widetilde Z_i\,. \label{channels}
	\end{cases}
\end{align} 
In the following we assume $\lambda = 1$, as it amounts to a scaling of $\bm{\Phi}$. Here $(\widetilde Z_i),(Z_\mu), (V_\mu)\iid \mathcal{N}(0,1)$ whereas $(X_i)\iid P_0$. The inference problem is to recover both $\bX=(X_i)_{i=1}^n$ and $\bV=(V_\mu)_{\mu=1}^m$ from the knowledge of the observations $\bY_t$, $\widetilde \bY_t$ and the matrix $\bm{\Phi}$ (and thus of $\bm{\Phi'}$ and $\bW$ too as the decomposition \eqref{eq:decomposition} is assumed to be known). 

In the Bayesian setting the posterior associated with this inference problem, written in the Gibbs-Boltzmann form, is
%
\begin{align}\label{post}
dP(\bx,\bv|\bY_t,\widetilde \bY_t,\bm{\Phi})=\frac{dP_0(\bx){\cal D}\bv e^{-{\cal H}(t,\bx,\bv;\bY_t,\widetilde \bY_t,\bm{\Phi})}}{\int dP_0(\bx){\cal D}\bv e^{-{\cal H}(t,\bx,\bv;\bY_t,\widetilde \bY_t,\bm{\Phi})}}\,,
\end{align}
%
where ${\cal D}\bv\equiv\prod_{\mu=1}^mdv_\mu (2\pi)^{-1/2}e^{-v_\mu^2/2}$ is the standard Gaussian measure, and we have defined the interpolating \emph{Hamiltonian} ${\cal H}={\cal H}(t,\bx,\bv;\bY_t,\widetilde \bY_t,\bm{\Phi})$ as
%
\begin{equation*}
\textstyle {\cal H}\equiv\frac12 \| \bY_t-\sqrt{\frac{1-t}{n}} \bm{\Phi}\bx\! -\! \sqrt{\frac{\widetilde E(t)}{n}} \bm{\Phi'} \bv \|_2^2 + \frac12 \| \widetilde \bY_t-\sqrt{rt}\,\bx \|_2^2\,,
\end{equation*}
%

It is a simple exercise (see e.g. \cite{barbier_ieee_replicaCS}) to show that the normalized mutual information $i_n(t)\equiv\frac1nI(\bX,\bV;\bY_t,\widetilde \bY_t|\bm{\Phi})$ for the interpolation estimation problem is related to the posterior normalization (or partition function) through 
\begin{equation}\label{eq:def_mutual_info}
\textstyle i_n(t)= -\frac{1}{n}\EE\ln \int dP_0(\bx) {\cal D}\bv e^{-{\cal H}(t,\bx,\bv;\bY_t,\widetilde \bY_t,\bm{\Phi})} -\frac{\alpha+1}{2}\,.
\end{equation}
%
This {\it interpolating mutual information} verifies
%
\begin{align}\label{i0i1}
\begin{cases}
		i_n(0)=i_n\,,\\
		i_n(1)=I(r)+\frac\alpha2 \EE_{X'} \ln (1 + \widetilde E(1) X')\,,
	\end{cases}	
\end{align}
%
where $X'\sim p'_n$, with $p'_n$ the empirical spectral distribution of the $m \times m$ matrix $\frac{1}{n}\bm{\Phi'}^\intercal \bm{\Phi'}$. The second term in the expression of $i_n(1)$ (sometimes refered to as a Shannon transform, see e.g. \cite{2004random}) is obtained using the celebrated ``log-det formula'' for the mutual information $\frac{1}{n}I(\bY_1;\bV|\bm{\Phi'})$ of an i.i.d. Gaussian input multiplied by the matrix $\bm{\Phi'}$ and under additive Gaussian noise, see e.g. \cite{2004random}.

Now a crucial step in our proof, that is a consequence of the particular form of the measurement matrix \eqref{eq:decomposition}, is that as $n$ grows, the second term in $i_n(1)$ can be replaced by an integrated R-transform:
%
\begin{align}\label{13}
\textstyle i_n(1)=I(r)+\frac12 \int_0^{\widetilde E(1)}  \mathcal{R}_{\bR}(-u) d u+ \smallO_n(1)\,,
% i_n(1)=I(X;\sqrt{r}X+Z)+\frac12  \int_0^E  \mathcal{R}_{\frac{1}{n}\bm{\Phi}^\intercal \bm{\Phi}}(-u) \mathrm{d} u +\frac12 + \smallO_n(1)
\end{align}
%
where $\mathcal{R}_{\bR}(z)$ is the R-transform associated with the asymptotic spectrum of $\bR=\frac{1}{n}\bm{\Phi}^\intercal \bm{\Phi}$. We give the definition of this transform as well as the proof of \eqref{13} in the next section.

\begin{remark}[A word about notations] We define the Gibbs Bracket $\langle-\rangle_t$ as the expectation w.r.t. the posterior \eqref{post}. In constrast, we denote by $\EE$ the joint expectation w.r.t. all \emph{quenched} variables (i.e. fixed by the realization of the problem), namely $\bY_t$ and $\widetilde \bY_t$, or equivalently w.r.t. $\bm{\Phi'}$, $\bW$, $\bX$, $\bV$, $\bZ$ and $\widetilde \bZ$.
\end{remark}

\subsection{Useful tools from random matrix theory}\label{sec:tools}
%
In this paragraph we show how to deduce \eqref{13} from \eqref{i0i1}. Note 
\begin{equation*}
\textstyle \mathbb{E}_{X'}\ln(1+\widetilde E(1) X') = \mathbb{E}_{X'}\int_0^{\widetilde E(1)} du \frac{X'}{1 + u X'}\,.
\end{equation*}
The result thus follows if the following relation is true :
\begin{equation}\label{R-S-relation}
\textstyle \mathcal{R}_{\bR} (- u) = \alpha \mathbb{E}_{X'}[\frac{X'}{1 + u X'}] +\smallO_n(1)\,.
\end{equation}
This is a well known relation in random matrix theory. For matrices of the form $\bR = \bW^\intercal \bT \bW$, where $\bW$ is a Gaussian $m\times n$ matrix with i.i.d. $\mathcal{N}(0, 1/n)$ elements, and $\bT=\frac{1}{n}\bm{\Phi'}^{\intercal}\bm{\Phi'}$ a non negative $m\times m$ matrix with a limiting spectral distribution, this was already shown by Marcenko and Pastur in 1967 \cite{marvcenko1967distribution} in the language of the Stieltjes transform. See also \cite{Silverstein-1995} for generalizations. Denoting by $g_\bR(z)$ and $g_\bT(z)$ ($z$ a complex number outside the 
specrum of the matrices)
the limiting Stieltjes transforms of the matrices $\bR$ and $\bT$, we have 
\cite{marvcenko1967distribution,Silverstein-1995} that the Marcenko-Pastur formula takes the form
\begin{align*}
\textstyle z (g_\bR(z))^2 + \alpha g_\bT( -1/g_\bR(z)) + (1-\alpha) g_\bR(z) = 0\,.
\end{align*}
Simple algebra then implies ($g_\bR^{-1}$ is the inverse function)
\begin{align*}
\textstyle g_\bR^{-1}(z) + z^{-1}  = - \alpha z^{-2} (g_\bT(-z^{-1}) - z)\,.
\end{align*}
Since by definition $\mathcal{R}_\bR(z) \equiv g_\bR^{-1}(-z) - z^{-1}$ and $g_\bT(z) \equiv \int  \frac{d\tau(x)}{x - z}$, $d\tau$ being the {\it limiting} 
eigenvalue distribution of $\bT$, this relation is nothing else than $\textstyle \mathcal{R}_\bR(-z) = \alpha \int  d\tau(x) \frac{x}{1 +zx}$
% \begin{align*}
% \textstyle \mathcal{R}_\bR(-z)   = \alpha \int  d\tau(x) \frac{x}{1 +zx}
% \end{align*}
which is equivalent to \eqref{R-S-relation} when $n\to\infty$. We refer to the review \cite{speicher2009free} for a more modern discussion using free probability concepts.

\subsection{Mutual information variation}
In order to ``compare'' the potential \eqref{replica} with the mutual information, we use the trivial identity $i_n = i_n(0) = i_n(1) -\int_0^1 i_n'(t) dt$ which becomes, using \eqref{13},
%
\begin{align}
	\textstyle i_n \!=\! I(r)+\frac12 \int_0^{\widetilde E(1)}  \mathcal{R}_{\bR}(-u) d u-\int_0^1 i_n'(t) dt+\smallO_n(1)\,. \label{14}
\end{align}
%The motivation in the introduction of the second term of the first channel and the second channel in \eqref{channels} is now apparent: Thanks to these, at $t=1$ the interpolating mutual information $i_n(1)$ has an expression very close to the potential which allows to ``construct'' it along the interpolation and obtain \eqref{14}.

We now evaluate $i_n'(t)$. Define $Q \equiv \frac{1}{n} \sum_{i=1}^n X_i x_i$, called the {\it overlap},
% \begin{align}
% Q &\equiv \frac{1}{n} \sum_{i=1}^n X_i x_i
% \end{align}
and the vector $\bu_{t}=(u_{t,\mu})_{\mu=1}^m$ with 
% $u_{t,\mu} \!\equiv\! [(1-t)/n]^{1/2}(\bm{\Phi}(\bX\! - \!\bx))_\mu\!+\! [\widetilde E(t)/n]^{1/2} (\bm{\Phi'}(\bV - \bv) )_\mu \!+\! Z_\mu$.
\begin{equation*}
\textstyle u_{t,\mu} \!\equiv\! \sqrt{\frac{1-t}{n}}(\bm{\Phi}(\bX\! - \!\bx))_\mu\!+\! \sqrt{\frac{\widetilde E(t)}{n}} (\bm{\Phi'}(\bV - \bv) )_\mu \!+\! Z_\mu\,.
\end{equation*}
%
% The goal of this subsection is to show the following lemma : 
% \textbf{FIXME : Fix the $\alpha$ factors in the case $\alpha \neq 1$...}
\begin{lemma}[Mutual information variation]\label{lemma:derivative}
For $t \in (0,1)$
\begin{align}
i_n'(t) = &~\frac{r}{2} (\rho - \EE \langle Q \rangle_t) + \smallO_n(1) \nn &+ \frac{1}{2n^2} \EE  \big\langle \bZ^\intercal (\bm{\Phi'} \bm{\Phi'}^\intercal) \bu_{t} [E(t) - (\rho - Q) ] \big\rangle_t\label{i'}
\end{align}
%
in which $\lim_{n\to\infty}\smallO_n(1)=0$ uniformly in $t \in (0,1)$.
\end{lemma}
%

The proof of this lemma, see \cite{proofAppendix}, is very similar to the one of Proposition 4 of \cite{Barbier2017}. The idea is to write explicitly the derivative $i_n'(t)$ and then to integrate by parts the quenched Gaussian variables $\bV$ and $\bW$, before using the {\it Nishimori identity}. This identity is a consequence of Bayes rule and the fact that we consider the {\it optimal Bayesian setting}, namely that all hyperparameters in the problem such as the snr and $P_0$ are known and used when defining the posterior, see \cite{barbier_stoInt,Barbier2017,REVIEWFLOANDLENKA}.

\subsection{Overlap concentration}

The next lemma essentially states that the overlap concentrates around its mean, and plays a key role in our proof. 
The proof technique for Bayesian 
inference has been developped in \cite{Macris2007,korada2010,korada2009exact,barbier_ieee_replicaCS} and is akin to the analysis reviewed for example in 
\cite{talagrand2010meanfield1}. The point however here is that in Bayesian inference overlap concentration can be proved in the whole phase diagram.
We will refer to \cite{barbier_stoInt,Barbier2017} where the analysis has been made quite generic. 

We introduce a ``small'' perturbation of the interpolating estimation problem by {\it adding} to the interpolating Hamiltonian $\cal H$ the term $\sum_{i=1}^n ( \epsilon x_i^2/2 - \epsilon x_i X_i - \sqrt{\epsilon} x_i \widehat{Z}_i)$
%
% \begin{align}\label{perturbation-ham}
% 	\sum_{i=1}^n \Big( \epsilon \frac{x_i^2}{2} - \epsilon x_i X_i - \sqrt{\epsilon} x_i \widehat{Z}_i \Big)
% \end{align}
%
where $(\widehat{Z}_i)_{i=1}^n \iid \mathcal{N}(0, 1)$.
This term can be interpreted as coming from a set of extra observations from a Gaussian side-channel $\widehat Y_i = \sqrt{\epsilon} X_i + \widehat{Z}_i$ for $i=1,\ldots,n$. Importantly this term
preserves the Nishimori identity. 
The new Hamiltonian defines a new Gibbs bracket $\langle - \rangle_{t, \epsilon}$ and interpolating mutual information $i_{n, \epsilon}(t)$. All the calculations of the previous section  trivially extend. 
This perturbation induces only a small change in the mutual information, namely of the order of $\epsilon$:
%
\begin{lemma}[Mutual information variation under perturbation]\label{lem:perturbation_f}
	Let $P_0$ with bounded support.
	For all $\epsilon > 0$ and all $t \in [0,1]$, $|i_{n,\epsilon}(t) - i_{n}(t) | = {\cal O}(\epsilon)$
	% \begin{align}
	% |i_{n,\epsilon}(t) - i_{n}(t) | = O(\epsilon) \,.	
	% \end{align}	
	where ${\cal O}(\epsilon)$ depends only on the size of the support of $P_0$, and on $\alpha$.
\end{lemma}
%
\begin{IEEEproof}
A computation using Gaussian integration by parts and the Nishimori identity gives 
$| \frac{\partial f_{n,\epsilon}(t)}{\partial \epsilon}|
= \frac{1}{2} | \mathbb{E} \langle Q \rangle_{t,\epsilon} |$.
\end{IEEEproof}
%

This small perturbation forces the overlap to concentrate:
%
\begin{lemma}[Overlap concentration] \label{concentration}
	For any $0\!<\! a \!< \!b \!<\!1$, $\lim_{n\to \infty}\int_{a}^b d\epsilon\int_0^1dt\, \mathbb{E}\langle (Q - \mathbb{E}\langle Q\rangle_{t, \epsilon})^2\ \rangle_{t, \epsilon}  = 0$.
	% \begin{align}
	% 	\lim_{n\to \infty}\int_{a}^b d\epsilon\int_0^1dt\, \mathbb{E}\big\langle \big(Q - \mathbb{E}\langle Q\rangle_{t, \epsilon}\big)^2\big \rangle_{t, \epsilon}  = 0\,.
	% \end{align}
\end{lemma}

We refer to \cite{barbier_stoInt,Barbier2017} for a detailed proof. As long as the concentration of the free energy of the interpolating model holds and that the unperturbed Hamiltonian 
satisfies the Nishimori identity (i.e., comes from a Bayesian inference probem) the analysis in \cite{barbier_stoInt,Barbier2017} applies verbatim. In other words the details 
of the unperturbed Hamiltonian do not matter. 
We stress that this lemma is the only place where the concentration of the free energy of the 
interpolating model is needed. For the present model under the assumptions on $\bm{\Phi'}$ this follows from Gaussian Poincar\'e and McDiarmid inequalities much as in \cite{Barbier2017}.

Note that the existence of the limit of the integrand in Lemma~\ref{concentration} as $n\to \infty$ is not known (and seems difficult to prove). Hence one cannot use Lebesgue's dominated convergence theorem to exchange the limit and 
the $\epsilon$-integral. However,
an elementary analysis argument based on the mean value theorem  shows the existence of a sequence $(\epsilon_n)_{n \geq 1}$ that converges to $0$ such that 
\begin{equation} \label{eq:int_overlap}
\textstyle \lim_{n\to\infty}\int_0^1dt \,
\EE\langle (Q - \mathbb{E}\langle Q\rangle_{t, \epsilon_n})^2\big \rangle_{t, \epsilon_n} =0\,.
\end{equation}
Note that Lemma~\ref{lem:perturbation_f} gives that $i_{n,\epsilon_n}(t)$ and $i_n(t)$ have same limit provided it exists.
In the next sections, in order to alleviate the notations in this short manuscript, we abusively remove 
the perturbation subscript $\epsilon_n$ since it makes no essential difference for the subsequent proofs but it is understood that all quantities are computed for 
the $\epsilon_n$-perturbed model.

\subsection{Upper and lower bounds}

This part is similar to parts 5.3 and 5.4 of \cite{Barbier2017}, or to what is done in \cite{2017arXiv170910368B}. As suggested by \eqref{i'}, in order to recover the potential on the r.h.s. of \eqref{14}, we want to choose for the interpolating function
\begin{align}\label{eq:equa_diff_E}
E(t) = \widetilde E'(t) = \rho - \EE \langle Q \rangle_t\,.
\end{align}
%
Note that \eqref{eq:equa_diff_E} is actually a first-order differential equation in $\widetilde E(t)$ ($\EE \langle Q \rangle_t$ is a function of $\widetilde E(t)$). Because $\EE \langle Q \rangle_t$ is a bounded $\mathcal{C}^1$ function of $(\widetilde E(t),r)$, the parametric Cauchy-Lipschitz theorem gives the following existence lemma.
\begin{lemma}[Optimal interpolation function]\label{lemma:cauchy_lipschitz}
Let $n \in \mathbb{N}^*$. For all $r \geq 0$, the differential equation \eqref{eq:equa_diff_E} admits a unique solution $E_n^{(r)}(t)\in[0,\rho]$. Moreover the mapping $r \in \mathbb{R}_+ \mapsto \int_0^1 E_n^{(r)}(s) ds\in [0,\rho]$ is continuous.
% \begin{align}
% \textstyle \widehat E_n : r \in \mathbb{R}_+ \mapsto \int_0^1 E_n^{(r)}(s) ds\,.
% \end{align}
\end{lemma}

We choose this optimal solution $E_n^{(r)}(t)$. We then apply the concentration \eqref{eq:int_overlap} for replacing the overlap by its mean $\EE\langle Q\rangle_t$ in \eqref{i'} under the integral in \eqref{14}. We use the Cauchy-Schwartz inequality to show that this is possible up to an $\smallO_n(1)$ correction. This leads to 
%
$\textstyle \int_0^1 i_n'(t)dt = (r/2)\int_0^1E_n^{(r)}(t)dt + \smallO_n(1)\,.$ 
Therefore \eqref{14} and \eqref{i'} allow to deduce the following.
%,{\color{blue} which forms the core of the proof, and that is obtained thanks to the choice of the optimal interpolation path permitted by the adaptive path interpolation.}
%
\begin{lemma}[Fundamental identity]\label{lemma:sequence}
Let $(r_n)_{n \in \mathbb{N}} \in \mathbb{R}_+^\mathbb{N}$ be a bounded sequence. 
%Denote $E_n^{(r_n)}(t) \equiv \Psi_n(r_n)'(t)$. 
Then 
\begin{equation}
\textstyle i_n = i_{\rm{RS}} (\int_0^1 E_n^{(r_n)}(s)ds,r_n) + \smallO_n(1)\,.\label{15}
\end{equation}
\end{lemma}
It immediately implies an upper bound:
\begin{proposition}[Upper bound] 
The mutual info. verifies
\begin{align}
\limsup_{n \to \infty} i_n \leq \inf_{r \geq 0} \sup_{E \in [0,\rho]} i_{\rm{RS}}(E,r)\,.
\end{align}
\end{proposition}
%
\begin{IEEEproof}
Choose a constant sequence $r_n=r$. Lemma~\ref{lemma:sequence} then implies $\limsup_{n\to\infty} i_n \le \sup_{E\in[0,\rho]}i_{\rm{RS}} (E,r)$. This is true for any $r\ge0$, therefore the result.	
\end{IEEEproof}
%

The lower bound is a bit more involved. Details of similar computations can be found in \cite{Barbier2017,2017arXiv170910368B}
\begin{proposition}[Lower bound] 
The mutual info. verifies
\begin{align}
\liminf_{n \to \infty} i_n \geq \inf_{r \geq 0} \sup_{E \in [0,\rho]} i_{\rm{RS}}(E,r)\,.
\end{align}
\end{proposition}
\begin{IEEEproof}
Note that due to our hypothesis and its consequence \eqref{R-S-relation}, the function $h : z \mapsto \mathcal{R}_{\bR}(-z)$ is a $\mathcal{C}^1$ function defined for all $z \geq 0$, and verifies $i)\ h(0) = \mathcal{R}_{\bR}(0)$ is finite; $ii)\ h'(z) < 0$ for all $z > 0$; and $iii) \ h(z) > 0$ for all $z > 0$.
% \begin{align*}
% h(0) &= \mathcal{R}_{\bm{\Phi}^\intercal \bm{\Phi}}(0) \text{ is finite} \\
% \forall z > 0 \quad &h'(z) < 0  \\
% \forall z > 0 \quad &h(z) > 0 
% \end{align*}

Define $K \equiv \max\left(\rho,h(0)\right)$. Then the mapping $r\in[0,K] \mapsto h(\int_0^1 E_n^{(r)}(t) dt)\in[0,K]$
% \begin{align*}
% [0,K] &\to [0,K] \\
% r &\mapsto h\left[\int_0^1 E_n^{(r)}(t) \mathrm{d}t\right]
% \end{align*}
is continuous by composition. It must thus admit a fixed point $r_n^*$.
It thus only remains to show 
\begin{equation}\label{eq:}
\textstyle i_{\rm{RS}}(\int_0^1 E_n^{(r_n^*)}(t) dt, r_n^*) = \sup_{E \in [0,\rho]} i_{\rm{RS}}(E,r_n^*)\,.
\end{equation}
This is true because at fixed $r$, the function $g_r(E) \equiv i_{\rm{RS}}(E,r)$ is strictly concave since $g_r''(E) = h'(E)/2 < 0$. The conclusion follows from the fact that the derivative can only vanish at the (achieved) maximum, and that $g_{r_n^*}'(\int_0^1 E_n^{(r_n^*)}(t) dt) = 0$; indeed this is the fixed point equation $r_n^*=h(\int_0^1 E_n^{(r_n^*)}(t)dt)$.

Finally \eqref{15} yields $i_n = \sup_{E \in [0,\rho]} i_{\rm{RS}}(E,r_n^*) + \smallO_n(1) \geq \inf_{r \geq 0} \sup_{E \in [0,\rho]} i_{\rm{RS}}(E,r) +\smallO_n(1)$, and thus the result.
% \begin{align}
% \textstyle i_n &= \sup_{E \in [0,\rho]} i_{\rm{RS}}(E,r_n^*) + \smallO_n(1) \nn
% \geq &\inf_{r \geq 0} \sup_{E \in [0,\rho]} i_{\rm{RS}}(E,r) +\smallO_n(1) 
% \end{align}
\end{IEEEproof}
%
%
% \subsection{Sketch of proof of Lemma~\ref{lemma:derivative}} \label{proofLemma}
% \input{short_proof_lemma3.1}

==> sections/results.tex <==
The random linear estimation problem with correlated, non i.i.d. matrices has been considered, again with the replica method, and a
solution was proposed by Takeda, Uda and Kabashima in the case of
CDMA \cite{TakedaUdaKabashima2006} for matrices taken from a {\it rotationally invariant ensemble}. The replica formula was
later extended by Tulino, Caire, Verdu and Shamai
\cite{tulino2013support} for such similar ensembles in order to allow for more complicated priors
such as Gauss-Bernoulli ones. These works point to a generic conjecture, that we now describe, giving the
single-letter formula for the mutual information.  

Consider a measurement matrix
$\bm{\Phi} = \bO \bm{\Sigma} \bN^\intercal$
% %
% \begin{align}\label{eq:decomposition_phi}
% \frac{1}{\sqrt{n}}\bm{\Phi} &= \bO \bm{\Sigma} \bN^\intercal \, ,
% \end{align}
where $\bO$ and $\bN$ are both orthogonal matrices and $\bm\Sigma$ is diagonal (non-square if $\alpha \neq 1)$. The matrices $\bm\Sigma$, $\bN$, $\bO$ are independent
and $\bN$ is distributed uniformly,
according to the \emph{Haar measure} of its orthogonal
group, in which case $\bm{\Phi}$ is said to be \emph{right-rotationally invariant} (if $\bO$ is also Haar distributed the ensemble is simply called rotationally invariant). The matrix 
$\bR\equiv \frac{1}{n}\bm{\Phi}^\intercal \bm{\Phi} = \frac{1}{n}\bN \bm{\Sigma}^\intercal\bm{\Sigma}\bN^\intercal$ plays an important role. For general rotationally invariant ensembles its eigenvalues are not necesssarily i.i.d. but typically
are such that
$\frac{1}{n}\bm{\Sigma}^\intercal\bm{\Sigma}$ has a suitable limiting eigenvalue distribution (as in fact assumed in \cite{TakedaUdaKabashima2006}). %A simpler model is to assume 
%$(\Sigma_{a a}^2)_{a=1}^{\min(m,n)}\iid p_{\bR}$ from a suitable given density distribution $p_\bR$.
% In \cite{tulino2013support} it is further assumed that the diagonal $m \times n$ matrix $\bm{\Sigma}$ is a
% independent of $\bO,\bN$ and taken with i.i.d. elements on its main diagonal
% from a given density distribution $p_\bR$ that we assume to be positively and compactly supported:
% $(\Sigma_{a a}^2)_{a=1}^{\min(m,n)} \iid p_{\bR}$ (in their case a Bernoulli distribution is assumed). However in \cite{TakedaUdaKabashima2006} it is only explicitly assumed that 
%  $\frac{1}{n}\bm{\Sigma}^\intercal\bm{\Sigma}$ has a limiting eigenvalue distribution (the $\Sigma_{a a}^2$ may not necessarily be i.i.d.).
The limit of the normalized mutual information is conjectured to be
% 
\begin{align}\label{conjecture}
\lim_{n\to\infty} i_n &=\sup_{(E,r)\in\Gamma}i_{\rm RS}(E,r;\lambda)
\end{align}
%
where the so-called replica symmetric {\it potential} $i_{\rm RS}(E,r;\lambda)=i_{\rm RS}$ is defined as
%
\begin{align}
\textstyle i_{\rm RS} \equiv
I(X;\sqrt{r}X+Z)+\frac{1}{2}\int_0^{E\lambda} {\cal R}_\bR(-z)dz -
\frac{rE}2 \,.  \label{replica}
\end{align}
Here we have used the \emph{R-transform} of the matrix $\bR$ (see \cite{2004random} for an introduction to such transforms). $I(X;\sqrt{r}X+Z)$, that we simply denote $I(r)$ later on, is the mutual information for 
the scalar Gaussian channel $Y=\sqrt{r}X+Z$, $X\sim P_0$ and $Z\sim{\cal N}(0,1)$. Moreover, $\Gamma$ is the
set of critical points of the potential, or \emph{state evolution}
fixed points ($\rho \equiv \EE_{P_0}[X^2]$)
%
\begin{align*}
\Gamma  \equiv \big\{(E,r)\in[0,\rho]\times \mathbb{R}_+\,\big|\, E&= {\rm mmse}(X|\sqrt{r}\,X+Z), \nn \quad r&=\lambda {\cal R}_\bR(-E\lambda)\big\}\,.
\end{align*}
%

A virtue of the formula \eqref{replica} is that the details of the rotation invariant matrix ensemble only enter through the R-transform.

Note the slight difference with the potential written in \cite{tulino2013support}: In the potential \eqref{replica} a factor $1/2$, not present in \cite{tulino2013support}, multiplies both the integrated R-transform and $-r E$. This is because they consider the 
complex $\bm{\Phi}$ case while we consider the real case (nevertheless, we believe that our proof techniques could easily be generalized to include the complex case).


Interestingly, Manoel {\it et al} \cite{Manoeletal} and Reeves
\cite{Reeves} were able to formally re-derive equivalent results independently
for a sub-class of rotationally invariant matrices by considering multi-layered
estimation problems. This line of work combined with our present rigorous work is giving a lot of credibility to the replica conjecture for the general rotation invariant ensemble.

\subsection{Main result}
Our main result is a proof of the replica conjecture
(\ref{conjecture}) for a specific, but large, set of correlated
matrices. We hope it paves the way towards a completely general proof, as the non-rigourous replica calculation only 
assumes right-rotational invariance of $\bm{\Phi}$. We assume that the $m \times n $ matrix $\bm{\Phi}$ can be decomposed as follows: 
\begin{align}\label{eq:decomposition}
\bm{\Phi} = \bm{\Phi'} \bW
\end{align}
in which all elements of the $m \times n$ matrix $\bW$ are i.i.d. 
Gaussians ${\cal N}(0,1/n)$ with mean zero and variance $1/n$, $\bm{\Phi'}$ is a $m\times m$ random matrix, and $\bW$, $\bm{\Phi'}$ are independent. 
Concerning $\bm{\Phi'}$, our analysis is currently complete under the assumption that it is a product of a finite number of independent matrices, each with 
i.i.d. matrix-elements that are either bounded or standard Gaussians. 
The case of a product of i.i.d. standard Gaussian matrices constitutes an interesting example
that has been considered in \cite{Manoeletal}.

Our goal here is to give a rigorous proof of
 \eqref{conjecture} in the setting of matrices \eqref{eq:decomposition} with the independence assumptions for $\bm{\Phi'}$. 
 Some of our technical calculations are based on previous related works, and all of them will be discussed in a complete manner in a longer contribution.
 %
\begin{theorem}[Replica formula]\label{thm:main_thm}
Assume that the prior $P_0$ has compact support or, in other words, the signal is bounded. Then with $n,m,\bm{\Phi},\bR,i_{\rm RS}$ defined as before (in particular $\bm{\Phi}$ satisfies \eqref{eq:decomposition} and the subsequent hypothesis), one has
\begin{align*}
\lim_{n\to\infty}i_n = \inf_{r\ge0}\sup_{E \in [0,\rho]}i_{\rm RS}(E,r;\lambda)\,.
\end{align*}
\end{theorem}
%
\begin{remark}[Equivalent expressions of the replica formula]
The right hand side in the theorem above can also be written as $\sup_{(E,r)\in\Gamma}i_{\rm RS}(E,r;\lambda)$ (if the extremizers are not attained at the boundaries, which is the case when noise is present) or as $\inf_{E \in [0,\rho]}\sup_{r\ge0}i_{\rm RS}(E,r;\lambda)$. A proof of such equivalences, in the case of generalized estimation, is found in \cite{Barbier2017}.
\end{remark}

\begin{remark}[Right-rotation invariance of the ensemble]
Note that \eqref{eq:decomposition} implies the right-rotation invariance of $\bm{\Phi}$ because of the rotation invariance of $\bW$. Our result thus covers a sub-class of right-rotationally invariant matrices. 
\end{remark}

\begin{remark}[Relaxing the assumptions on ${\bm \Phi'}$]
The assumptions on $\bm{\Phi'}$ come from the fact that a complete 
rigorous analysis requires proving the concentration of the ``free energy'' of an {\it interpolating} model (see below; the free energy is equal to the mutual information up to a trivial additive constant). 
This involves the use of tools such as the McDiarmid bounded difference inequality and/or the Gaussian Poincar\'e inequality, which require some independence between degrees of freedom. 
If one {\it assumes} concentration of the free energy of the interpolating model then one can relax these assumptions to the following more general ones.  
It then suffices to assume that $\frac{1}{n}\bm{\Phi'}^\intercal \bm{\Phi'}$ has a well-defined, positively and compactly supported, asymptotic 
eigenvalue distribution in the limit $n \to \infty$. We also remark that concentration proofs of the free energy of the original and interpolated models are technically similar, however we have not established a purely logical implication between the two.
If such an implication holds one could also replace the independence assumption on ${\bm{\Phi'}}$ by an assumption of concentration of the free energy. 
\end{remark}

\begin{remark}[Relaxing the assumption on $P_0$]
Boundedness of the signal is again used to obtain concentration results for the free energy but it can presumably be removed 
using a limiting argument as in \cite{MiolaneXX}.
\end{remark}

\subsection{Related works}
%
There has been a lot of effort recently
\cite{BarbierDMK16,barbier_ieee_replicaCS,ReevesPfister2016,Barbier2017}
to prove the Tanaka formula for random
i.i.d. matrices. Our strategy in the present paper is to follow the {\it adaptive
interpolation method} introduced in
\cite{barbier_stoInt,2017arXiv170910368B}. This method, in particular,
has been used by the authors of \cite{Barbier2017} to reach a rigorous
demonstration of the replica formula for the mutual
information for the case of i.i.d. measurement matrix $\bm{\Phi}$,
in the more general situation of ``generalized linear
estimation'' i.e.,  with an {\it arbitrary} measurement channel (instead of just
a random additive noise as in (\ref{eq:def_inference})).  Some
steps of our current approach consequently follow similar ones in
\cite{Barbier2017} (but with key differences) and we will refer to
this work when necessary. We believe, in fact, that the approach presented
in the present paper could further be generalized as well to
generalized linear estimation with rotationally invariant matrices to
reach the formula conjectured by Kabashima in
\cite{Kabashima2007}. This is left for future work. 

Perhaps the most important consequence of the replica formula is that
it predicts the value of the minimum mean-square error (MMSE) in the
reconstruction of the signal $\bX$. In fact, it is conjectured (and
proved for Gaussian matrices \cite{barbier_ieee_replicaCS,ReevesPfister2016}) to be given by the value $E$ that
extremizes \eqref{replica}. While we consider here mainly the
information theoretic result, a large body of work has focused on
algorithmic approaches to random linear estimation, and investigated
whether the MMSE is efficiently (say, in polynomial time)
achievable. 

For Gaussian matrices, the most successful approach, so far, again
originated in statistical physics
\cite{thouless1977solution,mezard1989space} and is called approximate
message-passing (AMP) \cite{donoho2009message}. AMP is Bayes-optimal
and efficiently achieves the MMSE for a large set of
parameters, as proven in \cite{barbier_ieee_replicaCS}. There, however, might exist a region called ``hard''
where this is not the case, and polynomial algorithms improving on AMP
are not known. Whether there exists an efficient algorithm that is able to beat AMP in the hard region is widely considered to be a notoriously difficult problem (see e.g. \cite{REVIEWFLOANDLENKA} and reference therein).

For rotationally invariant matrices, different but related approaches
were proposed \cite{TakedaUdaKabashima2006,SAMP}. In particular, the
general expectation-propagation (EP) \cite{Minka} leads to a powerful
scheme in this context \cite{EP}. Recently Ma and Ping proposed a
variation of EP called OAMP \cite{ma2017orthogonal} specially adapted
to these matrices. Rangan, Schniter and Fletcher introduced a related
approach called VAMP \cite{VAMP} and showed that it follows the fixed
point equation (called state evolution) of the potential
\eqref{replica}. Interestingly, the multi-layer AMP algorithm of
Manoel {\it et al.} \cite{Manoeletal} also has the same fixed
point. 
Our result thus supports that OAMP, VAMP (and multi-layer AMP)
are Bayes-optimal and efficiently reach the MMSE in the ``easy''
region of random linear estimation with these correlated matrices,
just as AMP does in the case of i.i.d. Gaussian matrices.




==> sections/setting__Copie_en_conflit_de_jean_barbier_2020-01-08_.tex <==
Let $\bX\in \mathbb{R}^{n \times d}$ an unknown random signal-matrix with prior distribution supported on a bounded interval ${\cal X}$ (independent of $n$) and that factorizes over the rows: $P_X=p_X^{\otimes n}$. Consider the observation model:
\begin{subequations}
\label{eq:general_model}
 \begin{alignat}{3}
\tilde \bY & = \bX S^{1/2} +\tilde \bW,\\
\bY_\ell & = n^{-1/2} \bX B_\ell \bX^\intercal +  \bW_\ell, \quad && \ell = 1, \dots, L,
\end{alignat}
\end{subequations}
where $S\in {\cal S}_d^+$, the set of $d\times d$ semidefinite positive matrices, and $\cB = \{ B_\ell\}_{\ell=1}^L$, $B_\ell \in \reals^{d \times d}$, are deterministically known. Instead $\tilde\bW$ and $\{\bW_\ell\}_{\ell=1}^L$ are independent noise matrices with i.i.d.\ standard Gaussian entries. Note that, by stability of the Gaussian law under addition, this model is equivalent to a model where the first channel in \eqref{eq:general_model} is replaced by $K$ independent Gaussian channels of the form $\tilde \bY_k= \bX A_k +\tilde \bW_k$ where $A_k\in\mathbb{R}^{d\times m_k}$. More precisely, this equivalence follows by setting $S=\sum_{k=1}^KA_kA_k^\intercal$, see , and by equivalence we mean that the Le Cam distance between the two models vanishes \cite{le2012asymptotic}, which implies mutual information and MMSE-wise equivalence.

Our analysis considers the regime $d,L$ (and $(m_k),K$ if considered) fixed while taking the thermodynamic limit $n\to +\infty$. We keep the bold notation for matrices with at least one dimension scaling with $n$. One could further generalize the model by considering additional higher-order tensor observations like $Y^{(p)}_{j,i_1\dots i_p}\!=\! n^{\frac{1-p}{2}} \sum_{k_1, \dots, k_p}^d \!C^{(p)}_{j,k_1 \dots k_p}X_{i_1k_1}\dots X_{i_pk_p} + W^{(p)}_{j,i_1\dots i_p}$ with $C^{(p)}_j$ an order-$p$ coupling tensor and $\bW_j^{(p)}$ an order-$p$ Gaussian noise tensor, with $p\ge 3$, $1\le j\le J$, $(i_1, \ldots, i_p)\in\{1,\ldots,n\}^p$. The analysis would be more involved notation-wise but would not present any additional difficulties, and is left for future work. The observation model \eqref{eq:general_model} encompasses a variety of matrix estimation problems. The most studied examples are the spiked Wigner model when taking $K=0$, $L=1$ and $B_1$ proportional to the $d$-dimensional identity. The spiked Wishart model, where one aims at recovering $\bU\in \reals^{n \times d}$ and $\bV \in \reals^{\alpha n \times d}$ from $\bY= \gamma n^{-1/2} \bU \bV^\intercal + \bW$, is found back as follows. Set $K=0$ and $L=1$. Without loss of generality assume $\alpha \le 1$. Introducing the $n \times 2d$ matrix $\bX = [\bU,\tilde{\bV}]$, where $\tilde{\bV}$ is obtained appending $n-\alpha n$ rows of zeros to $\bV$, and the $2d \times 2d$ matrix
\begin{align*}
B_1= \gamma\begin{bmatrix} 0_d &  {\rm I}_d \\  0_d &  0_d \end{bmatrix}, \ \text{then}\  \bX B_1 \bX^\intercal & =  \gamma \bU \tilde{\bV}^\intercal = \begin{bmatrix} \gamma \bU \bV^\intercal &  \boldsymbol{0} \end{bmatrix}.
\end{align*} 
Let us define 
\begin{align}
\cI_n(S,T)  & \equiv n^{-1}I\big(\bX;(\tilde \bY,\bY)\big)\label{eq:I_XW}
\end{align}
as well as $\bX_\ell \equiv \bX B_\ell \bX^\intercal$. Our main result reads:

\begin{theorem}[Replica symmetric formulas]
The mutual information for model \eqref{eq:general_model_alt} (and thus model \eqref{eq:general_model}) verifies
\begin{subequations}
\label{eq:RS}
\begin{alignat}{3}
	\lim_{n\to\infty}\cI_n(S,T)&={\adjustlimits \inf_{R\in {\cal S}^+_d} \sup_{Q\in{\cal S}^+_{d}}} {\cal I}(R,Q),\\
	{\cal I}(R,Q)&\equiv ??
\end{alignat}
\end{subequations}
As a consequence the generalized MMSE verifies
\begin{subequations}
\begin{align}
&\lim_{n\to\infty}\frac{1}{n^2}\mathbb{E} \|\bX_\ell -\mathbb{E}[\bX_\ell|\bY,\tilde \bY]\|_{\rm F}^2={\cal M}_\ell(R^*,Q^*)	\\
&{\cal M}_{\ell}(R,Q)\equiv ??
\end{align}
\end{subequations}
for any $(S,T)$ such that there exists a unique optimal couple $(R^*,Q^*)$ in the variational problem \eqref{eq:RS}.
\end{theorem}
